Semi-supervised Cycle-GAN for face photo-sketch translation in the wild

The performance of face photo-sketch translation has improved a lot thanks to deep neural networks. GAN based methods trained on paired images can produce high-quality results under laboratory settings. Such paired datasets are, however, often very small and lack diversity. Meanwhile, Cycle-GANs trained with unpaired photo-sketch datasets suffer from the \emph{steganography} phenomenon, which makes them not effective to face photos in the wild. In this paper, we introduce a semi-supervised approach with a noise-injection strategy, named Semi-Cycle-GAN (SCG), to tackle these problems. For the first problem, we propose a {\em pseudo sketch feature} representation for each input photo composed from a small reference set of photo-sketch pairs, and use the resulting {\em pseudo pairs} to supervise a photo-to-sketch generator $G_{p2s}$. The outputs of $G_{p2s}$ can in turn help to train a sketch-to-photo generator $G_{s2p}$ in a self-supervised manner. This allows us to train $G_{p2s}$ and $G_{s2p}$ using a small reference set of photo-sketch pairs together with a large face photo dataset (without ground-truth sketches). For the second problem, we show that the simple noise-injection strategy works well to alleviate the \emph{steganography} effect in SCG and helps to produce more reasonable sketch-to-photo results with less overfitting than fully supervised approaches. Experiments show that SCG achieves competitive performance on public benchmarks and superior results on photos in the wild.

==> tab_wildsketch.tex <==
\begin{table}[!t]
    \caption{\red{Quantitative comparison on WildSketch dataset.}}
    \label{tab:wildsketch}
    \centering
    \renewcommand{\arraystretch}{1.2}
    \small
    \begin{tabular}{c|*{6}{c}}
    \hline
         Method &  Cycle-GAN & GENRE & CA-GAN & PANet & Ours \\ \hline
         FSIM$\uparrow$ & 0.6654 & 0.6902 & \underline{0.6960} & 0.6950 & \textbf{0.7010} 
    \\ \hline
    \end{tabular}
\end{table}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{fig_wildsketch.png}
    \setlength{\tabcolsep}{0.em}
    \tiny
    \begin{tabularx}{\linewidth}{*{6}{C}}
    (a) Photo & (b) Cycle-GAN & (c) (S)CA-GAN & (d) PANet & (e) Ours & (f) GT \end{tabularx}
    \caption{\red{Example comparison with WildSketch dataset.}}
    \label{fig:wildsketch}
\end{figure}   
